The Firefly Sparkle: The Earliest Stages of the Assembly of A Milky Way-type Galaxy in a 600 Myr Old Universe

The most distant galaxies detected by JWST are assembling in a Universe that is less than 5\% of its present age. At these times, the progenitors of galaxies like the Milky Way are expected to be about 10,000 times less massive than they are now, with masses quite comparable to that of massive globular clusters seen in the local Universe. Composed today primarily of old stars and correlating with the properties of their parent dark matter halos, the first globular clusters are thought to have formed during the earliest stages of galaxy assembly. In this article we explore the connection between star clusters and galaxy assembly by showing JWST observations of a strongly lensed galaxy at zspec = 8.304, exhibiting a network of massive star clusters (the 'Firefly Sparkle') cocooned in a diffuse arc. The Firefly Sparkle exhibits the hallmarks expected of a future Milky Way-type galaxy captured during its earliest and most gas-rich stage of formation. The mass distribution of the galaxy seems to be concentrated in ten distinct clusters, with individual cluster masses that straddle the boundary between low-mass galaxies and high-mass globular clusters. The cluster ages suggest that they are gravitationally bound with star formation histories showing a recent starburst possibly triggered by the interaction with a companion galaxy at the same redshift at a projected distance of $\sim$2 kpc away from the Firefly Sparkle. The central star cluster shows nebular-dominated spectra consistent with high temperatures and a top-heavy initial mass function, the product of formation in a very metal poor environment. Combined with abundance matching that suggests that this is likely to be a progenitor of galaxies like our own, the Firefly Sparkle provides an unprecedented case study of a Milky Way-like galaxy in the earliest stages of its assembly in only a 600 million year old Universe.

==> interpretation.tex <==
\citep{papovich15} key paper for progenitor matching, finds MW progenitors out to z~3, lays out procedure that later papers use to go to even higher-z

\citep{graziani17} use the paper above to investigate a MW-like galaxy from z~20 to z~0. 

1979ARA&A..17..241H - bill harris MW GCs


How is this fundamentally different from the many papers in the literature by Dekel et al, Ceverino et al, Mandelker over the last decade? Maybe want to mention some of the works here: https://ui.adsabs.harvard.edu/abs/2017MNRAS.464..635M/abstract
https://ui.adsabs.harvard.edu/abs/2018ApJ...861..148M/abstract
https://academic.oup.com/mnras/article/443/4/3675/1010379


\citep{forbes20} linked 76 MW GCs to 5 progenitor satellite galaxies that have been accreted and subsequently disrupted. 

\citep{bournaud14} find long-lived clumps in high-z galaxy simulations that can migrate to the centers and survive for 100s of Myr

The \ffs represents one of JWST's first spectrophotometric observations of an extremely lensed galaxy assembling at high redshifts, and is especially interesting in context as a possible Milky-Way like progenitor. Abundance matching methods allow us to estimate the masses of galaxies that might be MW progenitors at high redshifts \citep{Behroozi:2013, papovich15}, and have been used to study the evolution of systems at high-z in both simulations and observations that can come to resemble our galaxy at late times \citep{papovich15, grazian17}. By comparing this against galaxies from the IllustrisTNG simulation \citep{pillepich19} or abundance matching using observed galaxy mass functions, we can estimate the range of stellar masses that a possible Milky Way or M31 progenitor can have at the redshift of the \ffs (detailed further in Section \ref{subsec:projmatch}). We find that the \ffs has a total mass of log M$_* \sim 6.8^{0.68}_{-0.26}$M$_\odot$, which is consistent with the mass we expect for a MW or M31-like galaxy in the present day universe. The implications of this are far reaching, but primarily that the \ffs could represent the early stages of a galaxy much like our own, unlike the extremely massive systems more commonly seen without lensing using JWST. 

We think of galaxies assembling at high-z in a very gas-rich environment \citep{papovich16} through accretion fueled starbursts, leading to disk formation \citep{2023BAAA...64..143I, 2015ApJ...808L..17F, 2024arXiv240200561N}. 
These gas-rich disks are subsequently disrupted or enhanced by mergers, instabilities, feedback, mis-aligned accretion and other events \citep{2016ASSL..418..355B, 2017MNRAS.464..635M, 2022MNRAS.512.3806V}.  
However, the current observations indicate that galaxy assembly at high redshifts occurs in a fundamentally different mode, with a majority of the stellar mass and SFR happening in dense gravitationally bound star clusters that seem to be stable against disruption by feedback (see section \ref{subsec:density_bound} for more details), or occurring in a regime where feedback is less effective \citep{2023MNRAS.523.3201D, 2024MNRAS.527.5929Y, 2023MNRAS.525L.117R}. The extreme conditions in these clusters can also alter the star formation efficiency and IMF, which can be tested with the current observations \citep{lancaster21}. This scenario is also favored by statistical studies \citep{2024MNRAS.527.5929Y}, which find that efficient stellar-driven winds (such as those arising from a top-heavy IMF or bursty star formation) could account for the self-consistent evolution of the galaxy mass function at high redshifts.
These `billiard balls' are sites of rapid star formation that may be stripped by tidal forces in the galaxy's nascent disk to become nuclear star clusters \citep{2016ASSL..418..355B, 2022ApJ...928..106T}. In particular, \citep{bournaud14} find in simulations that clumps can survive for $>100$ Myr because although they are being tidally stripped and losing mass, the gas-rich turbulent environment allows them to reaccrete gas at rates high enough to compensate for this. 
Another possibility is that some of these are ejected from the galaxy by mergers and other high-energy events and form the first generation of the galaxy's globular cluster population (Cluster 1 in this observation is a prime candidate for this). \citep{2015llg..book..477E, 2018RSPSA.47470616F} 
The \ffs provides a rich source for future observations that can test these scenarios to better understand the earliest stages of formation for galaxies like our own.

% (this section needs to be very well justified - and needs a ton of references)

--------

The standard model of structure formation suggests that galaxies form in the center of dark matter haloes due to inhomogeneities in the primordial mass distribution of the Universe. They grow by continuous accretion of gaseous material from the intergalactic medium, leading to an initial period of violent growth. This gas then settles into a rotationally-supported structure where stars are born, forming the stellar disc. The accretion of gaseous material onto the disc plays a crucial role in its evolution. At high redshifts, it is believed that the most massive galaxies were formed in intense nuclear starbursts and grew into the most massive local elliptical galaxies seen today, through mergers with minor companions.

--------

While the primary objective of this article is to highlight the \ffs object as a representative of high-z galaxy formation with both spatially resolved and spectrophotometric observations, with both the main galaxy and its companions having secure redshifts, it is important to note that the current analysis comes with several caveats. Changes in the magnification model as we further refine and add sources with future spectroscopic confirmations could change the estimated masses and magnifications of the clusters. However, the estimated t$_{50}$, sSFR, and surface densities are insensitive to this change and therefore do not change our overall picture. Additionally, given the extreme shear of this object it is unlikely that the magnification will significantly change from its current value. A second possible systematic is the modeling of the spectrophotometry, which could be affected by choices of stellar population and photoionisation models and assumed prior on parameters like the SFH, affecting estimates of stellar masses, IMF and star formation histories. The correct assumptions for these parameters and prior does not currently have consensus within the literature, but as JWST enables more observations at high redshifts we are gaining further insights into the possible systematics and accounting for them. In the current analysis, we have tried to mitigate the effects of these factors by adopting flexible non-parametric models where possible, and providing independent measurements where possible (e.g. for the electron temperature). We also find that these independent measurements tend to corroborate each other, e.g. the high electron temperature is consistent with scenarios with a top-heavy IMF \citep{Cameron2023}. Finally, a concern is that the absence of the rest-frame K-band makes estimating the stellar masses extremely fraught. While future MIRI observations will help definitively estimate the mass, our resolved analysis and non-parametric SFHs are expected to mitigate this effect \citep{sorba18,carnall19b, leja19} and provide a more robust estimate of the total mass of the system.  
